Explicit Computations of Fundamental Classes

We use the techniques of group cohomology to give explicit computations of the local fundamental class. As an application, we discuss how to compute the Tate canonical class for the extension $\mathbb Q(\zeta_{p^\nu})/\mathbb Q$, where $p^\nu$ is an odd prime power.

==> files/ntsetup.tex <==
Fix a finite abelian extension of local fields $L/K$. We will assume that $L/K$ is not unramified as a purely technical requirement; if $L/K$ is unramified, the extension is cyclic, so there are already computations of the fundamental class \cite[p.~102]{milne-cft}.

We now build the following tower of fields.
% https://q.uiver.app/?q=WzAsNixbMSwzLCJLIl0sWzAsMiwiS197XFxwaSxcXG51fSJdLFswLDEsIkwiXSxbMSwyLCJMXFxjYXAgTSJdLFsxLDEsIk0iXSxbMCwwLCJMTSJdLFswLDEsIlxcdGV4dHtyYW19IiwwLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsxLDIsIlxcdGV4dHt1bnJ9IiwwLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDMsIlxcdGV4dHt1bnJ9IiwyLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszLDIsIlxcdGV4dHtyYW19IiwyLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFszLDQsIlxcdGV4dHt1bnJ9IiwyLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyLDUsIlxcdGV4dHt1bnJ9IiwwLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDUsIlxcdGV4dHtyYW19IiwyLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dXQ==&macro_url=https%3A%2F%2Fraw.githubusercontent.com%2FdFoiler%2Fnotes%2Fmaster%2Fnir.tex
\[\begin{tikzcd}
	LM \\
	L & M \\
	{K_{\pi}} & {L\cap M} \\
	& K
	\arrow["{\text{ram}}", no head, from=4-2, to=3-1]
	\arrow["{\text{unr}}", no head, from=3-1, to=2-1]
	\arrow["{\text{unr}}"', no head, from=4-2, to=3-2]
	\arrow["{\text{ram}}"', no head, from=3-2, to=2-1]
	\arrow["{\text{unr}}"', no head, from=3-2, to=2-2]
	\arrow["{\text{unr}}", no head, from=2-1, to=1-1]
	\arrow["{\text{ram}}"', no head, from=2-2, to=1-1]
\end{tikzcd}\]
Unramified extensions have been labeled by ``unr,'' and totally ramified extensions have been labeled by ``ram.'' Here is the construction.
\begin{itemize}
    \item Set $n\coloneqq[L:K]$, and let $M$ be the unramified extension of $K$ of degree $n$. Note $\op{Gal}(M/K)$ is cyclic of order $n$ generated by the Frobenius automorphism $\sigma_K$. Extend $\sigma_K$ to an automorphism in $\op{Gal}(ML/K)$.
    \item Set $K_\pi\coloneqq(LM)^{\langle\sigma_K\rangle}$ so that $LM/K_\pi$ is unramified. Note $\op{Gal}(K/K_\pi)$ is a a finite abelian group, so we can write
    \[\op{Gal}(K/K_\pi)=\bigoplus_{i=1}^m\langle\sigma_i\rangle\]
    for some $\sigma_i\in\op{Gal}(K_\pi/K)$ of order $n_i$.
    \item Note $K_\pi$ is totally ramified over $K$, and $M$ is unramified over $K$, so $K_\pi$ and $M$ are linearly disjoint. Thus,
    \[\op{Gal}(LM/K)=\op{Gal}(M/K)\oplus\op{Gal}(K_\pi/K)=\langle\sigma_K\rangle\oplus\bigoplus_{i=1}^m\langle\sigma_i\rangle.\]
    Extend each $\sigma_i$ up to an automorphism of $LM$ accordingly.
    \item Set $f\coloneqq[L\cap M:K]$. Note $L\cap M$ is the maximal unramified subextension of $L$, so $\op{Gal}((L\cap M)/K)$ is cyclic generated by $\sigma_K|_{L\cap M}$ and is of order $f$. Because of the isomorphism $\op{Gal}(ML/L)\cong\op{Gal}(M/(L\cap M))$, we see that $\op{Gal}(ML/L)$ is cyclic of order $n/f$ generated by $\sigma_K^f$. It follows $L=(LM)^{\langle\sigma_K^f\rangle}$, so $K_\pi\subseteq L$, and
    \[\op{Gal}(L/K)=\frac{\op{Gal}(ML/K)}{\op{Gal}(ML/L)}=\langle\sigma_K|_L\rangle\oplus\bigoplus_{i=1}^m\langle\sigma_i\rangle,\]
    where the restriction $\sigma_K|_L$ has order $f$.
    \item Lastly, degree arguments or residue field computations can verify $LM/M$ and $L/(L\cap M)$ are all totally ramified extensions, though we will not need this.
\end{itemize}
For brevity, we will also set $G\coloneqq\op{Gal}(ML/K)$ and $H\coloneqq\op{Gal}(ML/L)$ so that $G/H=\op{Gal}(L/K)$.
% Then let $K_m$ be the largest unramified subextension, which we will give degree $m$; let $\overline\sigma_K\in\op{Gal}(L/K)$ denote the Frobenius automorphism, which lets us set
% \[K_{\pi,\nu}\coloneqq L^{\langle\overline\sigma_K\rangle}.\]
% In particular, $K_{\pi,\nu}/K$ is totally ramified because, for example, the residue fields of $K_{\pi,\nu}$ and $K$ have the same order.
% \begin{example}
% 	For $K=\QQ_p$, we can take $K_m=\QQ_p\left(\zeta_{p^m-1}\right)$ and $K_{\pi,\nu}=\QQ_p\left(\zeta_{p^\nu}\right)$.
% \end{example}
% This gives us the following tower of fields.
% % https://q.uiver.app/?q=WzAsNCxbMSwyLCJLIl0sWzAsMSwiS197XFxwaSxcXG51fSJdLFsyLDEsIktfbSJdLFsxLDAsIkwiXSxbMCwxLCIiLDAseyJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEsMywiIiwwLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFswLDIsIiIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMiwzLCIiLDIseyJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV1d&macro_url=https%3A%2F%2Fraw.githubusercontent.com%2FdFoiler%2Fnotes%2Fmaster%2Fnir.tex
% \[\begin{tikzcd}
% 	& L \\
% 	{K_{\pi,\nu}} && {K_m} \\
% 	& K
% 	\arrow[no head, from=3-2, to=2-1]
% 	\arrow[no head, from=2-1, to=1-2]
% 	\arrow[no head, from=3-2, to=2-3]
% 	\arrow[no head, from=2-3, to=1-2]
% \end{tikzcd}\]
% Quickly, we note that $L/K_{\pi,\nu}$ has Galois group generated by the Frobenius $\overline\sigma_K$ and therefore has degree $m$, so we have that $K_{\pi,\nu}$ and $K_m$ are linearly disjoint over $K$ and
% \[[L:K]=[L:K_{\pi,\nu}]\cdot[K_{\pi,\nu}:K]=[K_m:K]\cdot[K_{\pi,\nu}:K],\]
% which implies that $L=K_{\pi,\nu}K_m$ as well.

% We provide some quick commentary on these extensions.
% \begin{itemize}
% 	\item The extension $K_m/K$ is unramified of degree $f\coloneqq m$; note we are assuming $L\ne K_m$ and hence $f<n$. Its Galois group is thus generated by the Frobenius element defined by $\overline\sigma_K$.
% 	\item The extension $K_{\pi,\nu}/K$ is totally ramified of degree $[K_{\pi,\nu}:K]$. Because we are assuming this Galois group is abelian, we may write
% 	\[\op{Gal}(K_{\pi,\nu}/K)\simeq\Gamma_1\times\cdots\times\Gamma_t\]
% 	where $\Gamma_i=\langle\tau_i\rangle\subseteq\op{Gal}(K_{\pi,\nu}/K)$ is a cyclic group of order $n_i$.
% 	% Its Galois group is thus isomorphic to $\left(\ZZ/p^\nu\ZZ\right)^\times$, where the isomorphism takes $x\in\left(\ZZ/p^\nu\ZZ\right)^\times$ to
% 	% \[\sigma_x\colon\zeta_{p^\nu}\mapsto\zeta_{p^\nu}^{x^{-1}}.\]
% 	% The group $\left(\ZZ/p^\nu\ZZ\right)^\times$ is cyclic, so we will fix a generator $x$, which gives us a distinguished generator $\sigma_x\in\op{Gal}\left(\QQ(\zeta_{p^\nu})/\QQ_p\right)$.
% 	\item Because $K_{\pi,\nu}/K$ is totally ramified and $K_m/K$ is unramified, we have that the fields $K_{\pi,\nu}$ and $K_m$ are linearly disjoint over $K$. As such, $L=K_{\pi,\nu}K_m$ has
% 	\begin{align*}
% 		\op{Gal}(L/K_{\pi,\nu}) &\simeq \op{Gal}(K_m/K)=\langle\overline\sigma_K\rangle \\
% 		\op{Gal}(L/K_m) &\simeq \op{Gal}(K_{\pi,\nu}/K)=\Gamma_1\times\cdots\times\Gamma_t \\
% 		\op{Gal}(L/K) &\simeq \op{Gal}(K_m/K)\times\op{Gal}(K_{\pi,\nu}/K)=\langle\overline\sigma_K\rangle\times\Gamma_1\times\cdots\times\Gamma_t.
% 	\end{align*}
% 	In light of these isomorphisms, we will upgrade $\overline\sigma_K$ to the automorphism of $L/K$ which restricts properly on $K_m/K$ and fixing $K_{\pi,\nu}$; we do analogously for the $\tau_i$. We also acknowledge that our degree is
% 	\[n\coloneqq[L:K]=[K_m:K]\cdot[K_{\pi,\nu}:K]=f\cdot[K_{\pi,\nu}:K].\]
% \end{itemize}
% For brevity, we will also set $L_i\coloneqq L^{\langle\tau_i\rangle}$ for each $i$, which makes the fields under $L$ look like the following.
% % https://q.uiver.app/?q=WzAsNyxbMSwzLCJLIl0sWzIsMiwiS19tIl0sWzAsMSwiTF8wPUtfe1xccGksXFxudX0iXSxbMSwwLCJMIl0sWzIsMSwiTF8xIl0sWzMsMSwiXFxjZG90cyJdLFs0LDEsIkxfdCJdLFswLDEsIiIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMiwzLCIiLDAseyJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsMiwiIiwwLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs0LDMsIiIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMSw0LCIiLDIseyJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzEsNiwiIiwyLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFs2LDMsIiIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=&macro_url=https%3A%2F%2Fraw.githubusercontent.com%2FdFoiler%2Fnotes%2Fmaster%2Fnir.tex
% \[\begin{tikzcd}
% 	& L \\
% 	{K_{\pi,\nu}} && {L_1} & \cdots & {L_t} \\
% 	&& {K_m} \\
% 	& K
% 	\arrow[no head, from=4-2, to=3-3]
% 	\arrow[no head, from=2-1, to=1-2]
% 	\arrow[no head, from=4-2, to=2-1]
% 	\arrow[no head, from=2-3, to=1-2]
% 	\arrow[no head, from=3-3, to=2-3]
% 	\arrow[no head, from=3-3, to=2-5]
% 	\arrow[no head, from=2-5, to=1-2]
% \end{tikzcd}\]
% In particular, $\op{Gal}(L/L_i)=\langle\tau_i\rangle$ is cyclic for each $i$.

% Now, the main idea in the computation is to use an unramified extension $M\coloneqq K_n$ of the same degree $n$ as $L/K$. This modifies our diagram of fields as follows.
% % https://q.uiver.app/?q=WzAsNixbMSwzLCJLIl0sWzAsMiwiS197XFxwaSxcXG51fSJdLFsxLDAsIk1MIl0sWzAsMSwiTCJdLFsxLDIsIktfbSJdLFsyLDEsIk0iXSxbMCwxLCJcXHRleHR7cmFtfSIsMCx7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMSwzLCJcXHRleHR7dW5yfSIsMCx7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCw0LCJcXHRleHR7dW5yfSIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCw1LCJcXHRleHR7dW5yfSIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMywyLCJcXHRleHR7dW5yfSIsMCx7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNSwyLCJcXHRleHR7cmFtfSIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCwzLCJcXHRleHR7cmFtfSIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=&macro_url=https%3A%2F%2Fraw.githubusercontent.com%2FdFoiler%2Fnotes%2Fmaster%2Fnir.tex
% \[\begin{tikzcd}
% 	& ML \\
% 	L && M \\
% 	{K_{\pi,\nu}} & {K_m} \\
% 	& K
% 	\arrow["{\text{ram}}", no head, from=4-2, to=3-1]
% 	\arrow["{\text{unr}}", no head, from=3-1, to=2-1]
% 	\arrow["{\text{unr}}"', no head, from=4-2, to=3-2]
% 	\arrow["{\text{unr}}"', no head, from=3-2, to=2-3]
% 	\arrow["{\text{unr}}", no head, from=2-1, to=1-2]
% 	\arrow["{\text{ram}}"', no head, from=2-3, to=1-2]
% 	\arrow["{\text{ram}}"', no head, from=3-2, to=2-1]
% \end{tikzcd}\]
% We have labeled the unramified extensions by ``$\textrm{unr}$'' and the totally ramified extensions by ``$\textrm{ram}$.''

% % For brevity, we set $K\coloneqq\QQ_p$ and $L\coloneqq\QQ_p(\zeta_N)$ and $M\coloneqq\QQ_p(\zeta_{N'})$ so that $ML=\QQ_p(\zeta_N,\zeta_{N'})$. This abbreviates our diagram into the following.
% % % https://q.uiver.app/?q=WzAsNCxbMSwzLCJLIl0sWzAsMSwiTCJdLFsyLDEsIk0iXSxbMSwwLCJNTCJdLFsxLDMsIiIsMCx7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCwxLCIiLDAseyJzdHlsZSI6eyJoZWFkIjp7Im5hbWUiOiJub25lIn19fV0sWzAsMiwiIiwyLHsic3R5bGUiOnsiaGVhZCI6eyJuYW1lIjoibm9uZSJ9fX1dLFsyLDMsIiIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XV0=&macro_url=https%3A%2F%2Fraw.githubusercontent.com%2FdFoiler%2Fnotes%2Fmaster%2Fnir.tex
% % \[\begin{tikzcd}
% % 	& ML \\
% % 	L && M \\
% % 	\\
% % 	& K
% % 	\arrow[no head, from=2-1, to=1-2]
% % 	\arrow[no head, from=4-2, to=2-1]
% % 	\arrow[no head, from=4-2, to=2-3]
% % 	\arrow[no head, from=2-3, to=1-2]
% % \end{tikzcd}\]
% As before, we provide some comments on the field extensions.
% \begin{itemize}
% 	\item The extension $M/K$ is unramified of degree $n$. As before, its Galois group is cyclic, generated by the Frobenius element $\sigma_K\in\op{Gal}(M/K)$. Observe that $\sigma_K$ restricted to $K_m$ is $\overline\sigma_K$, explaining our notation. In particular, $\sigma_K$ has order $n$, but $\overline\sigma_K$ has order $f<n$.
% 	\item As before, note that $K_{\pi,\nu}$ and $M$ are linearly disjoint over $K$ because $K_{\pi,\nu}/K$ is totally ramified while $M/K$ is unramified. As such, we may say that
% 	\begin{align*}
% 		\op{Gal}(ML/M) &\simeq \op{Gal}(K_{\pi,\nu}/K) = \Gamma_1\times\cdots\times\Gamma_t \\
% 		\op{Gal}(ML/K_{\pi,\nu}) &\simeq \op{Gal}(M/K) = \langle\sigma_K\rangle \\
% 		\op{Gal}(ML/K) &\simeq \op{Gal}(M/K)\times\op{Gal}(K_{\pi,\nu}/K) = \langle\sigma_K\rangle\times\Gamma_1\times\cdots\times\Gamma_t.
% 	\end{align*}
% 	Again, we will upgrade $\sigma_K$ and the $\tau_i$ to their corresponding automorphisms on any subfield of $ML$.
% 	\item We take a moment to compute
% 	\begin{align*}
% 		\op{Gal}(ML/L) &\simeq \left\{\sigma_K^{a}\tau\in\op{Gal}(ML/K):\sigma_K^{a}\tau|_L=\id_L\right\}.
% 	\end{align*}
% 	Because $L$ is $K_{\pi,\nu}K_m$, it suffices to fix each of these fields individually. Well, to fix $K_{\pi,\nu}$, we need $\tau$ to vanish, so we might as well force $\tau=1$. But to fix $K_m$, we need $\sigma_K^{a}|_{K_m}=\overline\sigma_K^{a}$ to be the identity, so we are actually requiring that $f\mid a$ here. As such,
% 	\[\op{Gal}(ML/L)=\langle\sigma_K^f\rangle.\]
% \end{itemize}
% These comments complete the Galois-theoretic portion of the analysis.

% \subsection{Idea}
% We will begin by briefly describe the outline for the computation. For a finite extension of local fields $L/K$, let $u_{L/K}\in H^2(L/K)$ denote the fundamental class.

% Now, take variables as in our set-up in \autoref{sec:setup}. The main idea is to translate what we know about the unramified extension $M/K$ over to the general extension $L/K$. In particular, we are able to compute the fundamental class $u_{M/K}\in H^2(M/K)$, so we observe that
% % , by \autoref{prop:functorialfundclass},
% \[\op{Inf}_{M/K}^{ML/K}u_{M/K}=[ML:M]u_{M/K}=n\cdot u_{ML/K}=[ML:L]u_{ML/L}=\op{Inf}_{L/K}^{ML/K}u_{L/K}.\]
% As such, we will be able to compute $u_{L/K}$ as long as we are able to invert the inflation map $\op{Inf}\colon H^2(L/K)\to H^2(ML/K)$. This is not actually very easy to do in general, but we are in luck because this inflation map here comes from the Inflation--Restriction exact sequence
% \[0\to H^2(L/K)\stackrel{\op{Inf}}\to H^2(ML/K)\stackrel{\op{Res}}\to H^2(ML/L).\]
% The argument for the Inflation--Restriction exact sequence is an explicit computation on cocycles (involving some dimension shifting), but it can be tracked backwards to give the desired cocycle.
